MT* : Multi-Robot Path Planning for Temporal Logic Specifications

We address the path planning problem for a team of robots satisfying a complex high-level mission specification given in the form of an Linear Temporal Logic (LTL) formula. The state-of-the-art approach to this problem employs the automata-theoretic model checking technique to solve this problem. This approach involves computation of a product graph of the Buchi automaton generated from the LTL specification and a joint transition system which captures the collective motion of the robots and then computation of the shortest path using Dijkstra's shortest path algorithm. We propose MT*, an algorithm that reduces the computation burden for generating such plans for multi-robot systems significantly. Our approach generates a reduced version of the product graph without computing the complete joint transition system, which is computationally expensive. It then divides the complete mission specification among the participating robots and generates the trajectories for the individual robots independently. Our approach demonstrates substantial speedup in terms of computation time over the state-of-the-art approach, and unlike the state of the art approach, scales well with both the number of robots and the size of the workspace

==> Images/intro.tex <==
\section{Introduction} 
\label{sec-introduction} 
Motion planning is one of the core problems in robotics where we design algorithms to enable autonomous robots to carry out a real-world complex task successfully~\cite{LaValle:2006:PA:1213331}. A basic motion planning task consists of point-to-point navigation while avoiding obstacles and satisfying some user-given constraints. To solve this problem, there exist many methods among which
graph search algorithms like \textsf{A*}~\cite{Astar4082128} and sampling based motion planning techniques such as rapidly exploring random trees~\cite{doi:10.1177/02783640122067453} are two prominent ones.
Recently, there has been an increased interest in specifying complex motion plans using temporal logic (e.g.~\cite{Kress-GazitFP07,KaramanF09,BhatiaKV10,WongpiromsarnTM12,ChenTB12,UlusoySDBR13,SahaRKPS14}).
Using temporal logic~\cite{Baier:2008:PMC:1373322}, one can specify requirements that involve temporal relationship between different operations performed by robots.
%Such requirements arise in many robotic applications, including persistent surveillance~\cite{UlusoySDBR13}, assembly planning~\cite{Halperin1998}, 
%evacuation~\cite{RodriguezA10}, search and rescue~\cite{Jennings97}, localization~\cite{Fox00}, object transportation~\cite{Rus95}, and formation control~\cite{Balch98}.

A number of algorithms exist for solving Linear Temporal logic (LTL) motion planning problems in different settings (e.g~\cite{sampling5509503},~\cite{Kantaros2017},~\cite{VasileB13},~\cite{belta5650896},~\cite{UlusoySDBR13}). For an exhaustive review on this topics, the readers are directed to the survey by Plaku and Karaman~\cite{PlakuK15}.
% Several prior work considers a subset of LTL, either co-safe LTL or LTL over finite trace (LTL-f), where a finite trajectory can be synthesized to satisfy the specifications. 
In this paper, we focus on the class of multi-robot LTL motion planning problems where the robots have \emph{discrete dynamics} and the specification requires the robots to repeat some tasks perpetually. 
Such requirements arise in many robotic applications, including persistent surveillance~\cite{UlusoySDBR13}, assembly planning~\cite{Halperin1998}, 
evacuation~\cite{RodriguezA10}, search and rescue~\cite{Jennings97}, localization~\cite{Fox00}, object transportation~\cite{Rus95}, and formation control~\cite{Balch98}.
Traditionally, the LTL motion planning problem for the robots with discrete dynamics is reduced to the problem of finding the shortest path in a weighted graph and Dijkstra's shortest path algorithm~\cite{Cormen:2009:IAT:1614191} is employed to generate an optimal trajectory satisfying an LTL query~\cite{belta5650896,UlusoySDBR13}. 
However, for a large workspaces and a complex LTL specification, this approach is merely scalable.
We seek to design a computationally efficient algorithm to generate optimal trajectories for the robots. 

% Heuristics based search algorithms such as \textsf{A*}~\cite{Russell:2009:AIM:1671238} have been successfully used in solving point-to-point motion planning problems and is proven to be significantly faster than Dijkstra's shortest path algorithm.
Heuristic based search algorithms such as A* (for a single robot)~\cite{Russell:2009:AIM:1671238} and M* (for a multi-robot system)~\cite{WAGNER20151} have been successfully applied to solving point-to-point path planning problems and are proven to be significantly faster than Dijkstra's shortest path algorithm. Heuristic search based algorithms have also been applied to solving the temporal logic path planning problem for a single robot~\cite{BacchusK98,BaierM06a,BaierM06b,PatriziLGG11,KhalidiGS20}.
% \textsf{A*} algorithm has not been applied to temporal logic path planning as there is no notion of a single destination state in LTL motion planning. 
In this paper, we introduce the \textsf{MT*} algorithm that for the first time attempts to incorporate the heuristic search in LTL path planning to generate an \emph{optimal} trajectory for a multi-robot system satisfying an LTL query efficiently. 
We apply our algorithm to solving various LTL motion planning problems for a multi-robot system in 2-D workspaces and compared the results with that of the algorithm presented in~\cite{UlusoySDBR13}.
Our experimental results demonstrate that \textsf{MT*} in many cases achieves an order of magnitude better computation time than that of the traditional approach~\cite{UlusoySDBR13} to solve LTL motion planning problems.

\textsf{MT*} is a special class of multi-agent path finding (MAPF) problem.
MAPF is a widely studied planning problem where the goal is to find collision-free paths for a number of agents from their initial locations to some specified goal locations~\cite{MaK17}. MAPF is a special class of the finite LTL path synthesis problem~\cite{sampling5509503,CamachoBMM18} for multi-agent systems where the specification of each robot is given by the LTL formula ``eventually $goal$'', where $goal$ is the proposition that becomes true when all the robots reach their goal locations. On the contrary, our focus in the paper is to address the planning problem for those LTL specifications that capture perpetual behavior and is satisfied using infinite trajectories, like the work presented in ~\cite{belta5650896} and~\cite{KantarosZ19}.
Though the work by Kantaros and Zavlanos~\cite{KantarosZ19} scales for a large number of robots by using sampling based technique to compute first feasible trajectory(which might not have minimum cost), unlike their work, we focus on generating trajectories with minimum cost. 
%, our focus in this paper is rather those LTL specifications that can be satisfied only by infinite trajectories represented by a prefix followed by a loop.



==> Images/prelim.tex <==

\section{Preliminaries} % Main chapter title
\label{sec-preliminaries}


\subsection{Workspace, Robot Actions and Trajectory}
% The environments for robotic applications are continuous in nature. To reduce the amount of computation required during the motion planning of the robots in such environments, they are partitioned %discredited 
% into smaller cells or blocks based on the dynamics of the robot. We call it a \emph{discrete workspace} in this paper.
In this paper, we assume that a team of $n$ robots operates in a 2-D or a 3-D discrete workspace $\mathcal{W}$ which we represent as a grid map. The grid divides the workspace into square shaped cells. Every cell in the workspace $\mathcal{W}$ can be  referenced using its coordinates. Some cells in the grid can be marked as obstacles and cannot be visited by any robot. We denote set of obstacles using $\mathcal{O}$.
We capture the motion of a robot using  a set of actions $Act$. The robot changes its state in the workspace by performing the actions from $Act$. An action $act \in Act$ is associated with a $cost$ which captures the energy consumption or time delay (based on the need) to execute it. A robot can move to satisfy a given specification by executing a sequence of actions in $Act$ generating a \emph{trajectory} of states it attains. The \emph{cost of a trajectory} is the sum of costs of the actions to generate the trajectory. 

\subsection{Transition System}
We model the motion of the robot $i$ in the workspace $\mathcal{W}$ as a weighted transition system defined as
{
$\displaystyle
\begin{aligned}[c] 
\hspace{2cm} T^i := (S^i, s_0^i, E^i,\Pi^i, L^i, w^i)
\end{aligned}
$ 
\par}
% $T^i := (S^i, s_0^i, E^i,\Pi^i, L^i, w^i, \mathcal{O}^i )$ 
\noindent where (i) $S^i$ is the set of states,  
(ii) $s_0^i \in S^i$ is the initial state of the robot $i$,  (iii) $E^i \subseteq S^i \times S^i$ is the set of transitions/edges allowed to be taken by robot $i$, $(s_1^i , s_2^i) \in E^i$  iff  $s_1^i , s_2^i \in S^i$ and $s_1^i$ $\xrightarrow[]{act}$ $s_2^i$, where $act \in Act$,  (iv) $\Pi^i$ is the set of atomic propositions defined for robot $i$, (v) $L^i : S^i$ $\rightarrow$ $2^{\Pi^i}$ is a map which provides the set of atomic propositions satisfied at a state, (vi) $w^i: E^i$ $\rightarrow$ $\mathbb{N}_{>0}$ is a weight function.

%\is{The set of obstacles should not be part of the transition system of a robot.}\dg{Done}

\subsection{Joint Transition System}
A joint transition system $T$ is a transition system which captures the collective motion of a team of $n$ robots in a workspace$(\mathcal{W})$, where each robot executes one action from the set of actions $Act$ available to it. We define a joint transition system as
{
$\displaystyle
\begin{aligned}
    \hspace{2cm} T :=\: ( S_T,\; s_0,\; E_T,\; \Pi_T,\; L_T,\; w_T ),
\end{aligned}
$ 
\par}
% $T :=\: ( S_T,\; s_0,\; E_T,\; \Pi_T,\; L_T,\; w_T )$
\noindent where (i) $S_T$ is the set of vertices/states in a joint transition system, where each vertex is of form $\langle s^1, s^2,...,s^n\rangle$, $s^i$ represents the state of robot $i$ in transition system $T^i$, (ii) $s_0:=\langle s^1_0, s^2_0,...,s^n_0\rangle  \in S_T$ is the joint initial state of the team of $n$ robots, (iii) $E_T \subseteq S_T \times S_T$ is the set of edges. $(s_1,s_2) \in E_T$ iff $s_1 , s_2 \in S_T$ and $(s_1^i,s_2^i) \in E^i$ for all $i \in \{ 1,2,...,n\}$, (iv) $\Pi^T := \bigcup_{i=1}^n \Pi^{i}$ is the set of atomic propositions, (v) $L_T :  S_T \rightarrow 2^{\Pi_T}$, and $L_T(s_{1}) := \bigcup_{i=1}^n L^i(s_{1}^i)$ gives us set of propositions true at state $s_1$, (vi) $w_T : E^T \rightarrow \mathbb{N}_{>0}$, and $w_T( s_{1}, s_{2} ) := \sum_{i=1}^n w^i(s_{1}^i, s_{2}^i)$ is a weight function.

We can also think of the transition system as a weighted directed graph with vertices, edges and a weight function. So, whenever we use some graph algorithm over a transition system, we mean to apply it over it's equivalent graph. 


\begin{figure}[h] 
\centering
\subfigure[Workspace $\mathcal{W}$ with propositions $P_{1}, P_2 \text{ and } P_{3} $]{\centering \label{exampleGrid}\includegraphics[width=40mm]{Images/Workspace.png}}
\hspace{2mm}
\subfigure[B\"{u}chi automaton B for query: $\square(\Diamond P_{1} \land \Diamond P_{2} \land \lnot P_{3})$]{\centering \label{exampleAutomata}\includegraphics[width=37mm]{Images/Autometa.png}}
\caption{Workspace $\mathcal{W}$ and B\"uchi Automaton}
\label{ws}
\end{figure}

\begin{example}
Throughout this paper, we will use a warehouse pick-and-drop example for the illustration purpose.
%Throughout this paper, we will use the workspace $\mathcal{W}$ shown in Figure \ref{exampleGrid} for the illustration purpose. 
The workspace $\mathcal{W}$ is shown in Figure \ref{exampleGrid}. 
We build a transition systems $T^i$ for all the robots over $\mathcal{W}$ where $\Pi^i = \Pi_T = \{ P_1, P_2 , P_3 \}$. The proposition $P_i$ is satisfied if the robot is at one of the locations denoted by $P_i$.
Here, $P_1$, $P_2$ and $P_3$ correspond to drop location, pickup location, and the locations to be avoided by the robots, respectively. Cells with black colour represent obstacles ($\mathcal{O}$).
We assume that, from any cell in $\mathcal{W}$, a robot can move to one of its four neighbouring cells with cost 1 or stay at the same location with cost 0. 
\end{example}

\subsection{Linear Temporal Logic}
The motion planning query/task in our work is given in terms of formulas written using \emph{Linear Temporal Logic} (LTL).
\sloppy{LTL formulae over the set of atomic propositions $\Pi_T$ are formed according to the following grammar~\cite{Baier:2008:PMC:1373322}:
{
$\displaystyle
\begin{aligned}[c] 
    \hspace{1cm} \Phi:: = \mathtt{true} \;|\; a \;| \;\phi_{1} \land \phi_{2} \;|\; \neg\phi \;|\; X \phi \;|\; \phi_{1} U \phi_{2}.
\end{aligned}
$ 
\par}
% $$\Phi:: = \mathtt{true} \;|\; a \;| \;\phi_{1} \land \phi_{2} \;|\; \neg\phi \;|\; X \phi \;|\; \phi_{1} U \phi_{2} $$ 
The basic ingredients of an LTL formulae are the atomic propositions $a \in \Pi_T$, the Boolean connectors like conjunction $\land$ and negation $\neg$, and two temporal operators $X$ (next) and $U$ (until). 
The semantics of an LTL formula is defined over an infinite trajectory $\sigma$. 
The trajectory $\sigma$ satisfies a formula $\xi$, if the first state of $\sigma$ satisfies $\xi$.
The logical operators conjunction $\land$ and negation $\neg$ have their usual meaning.
For an LTL formula $\phi$,
$X\phi$ is $\textsf{true}$ in a state if $\phi$ is satisfied at the next step. The formula $\phi_1 \ U \ \phi_2$ denotes that $\phi_1$ must remain $\textsf{true}$ until $\phi_2$ becomes $\textsf{true}$ at some point in future.
The other LTL operators that can be derived are  $\square$ (\emph{Always}) and $\Diamond$ (\emph{Eventually}). The formula $\square \phi$ denotes that $\phi$ must be satisfied all the time in the future. The formula $\Diamond \phi$ denotes that $\phi$ has to hold sometime in the future. We have denoted negation $\lnot P$ as $!P$ and conjunction as $\&$ in the Figures. }

\subsection{B{\"u}chi Automaton}
For any LTL formulae $\Phi$ over a set of propositions $\Pi_T$, we can construct a B{\"u}chi automaton with input alphabet $\Pi_B = 2^{\Pi_T}$. We can define a B{\"u}chi automaton as
{
$\displaystyle
\begin{aligned} 
    \hspace{2cm} {B:= (Q_B, q_0, \Pi_B, \delta_B, Q_f)},
\end{aligned}
$ \par}
% ${B:= (Q_B, q_0, \Pi_B, \delta_B, Q_f)}$, 
\noindent where (i) $Q_B$ is a finite set of states, (ii) $q_0 \in Q_B$ is the initial state, (iii) $\Pi_B = 2^{\Pi_T}$ is the set of input symbols accepted by the automaton, (iv) $\delta_B \subseteq Q_B \times \Pi_B \times Q_B$ is a transition relation, and (v) $Q_f \subseteq Q_B$ is a set of final states.
An accepting state in the B\"uchi automaton is the one that needs to occur infinitely often on an infinite length string consisting of symbols from $\Pi_B$ to get accepted.
\begin{example}
Figure \ref{exampleAutomata} shows the B\"uchi automaton for an LTL task $\square(\Diamond P_{1} \land \Diamond P_{2} \land \neg P_{3})$, which captures the requirement that the robots should always repeat visiting pick up locations $P_2$ and drop location $P_1$, and always avoid locations $P_3$. Here, $q_0$ is the start state as well as the final state. It informally depicts the steps to be followed in order to compete the task $\Phi$. The transitions $q_1 \rightarrow q_2 \rightarrow q_0$ leads us to visit a state 
where $P_1 \land \lnot P_2 \land \lnot P_3$ is satisfied by going through only those states which satisfy $\lnot P_1 \land \lnot P_3$ and then go to state where $P_2 \land \lnot P_3 $ is satisfied using states which  satisfy $\lnot P_2 \land \lnot P_3$. This way, we can also understand the meaning of the other transitions. 
% \dg{As per the analogy we used above, this LTL mission tell the robots to always and eventually visit pick up locations $P_2$ and drop location $P_1$ and always avoid locations $P_3$.}    
\subsection{Product Automaton}\label{productAutomaton}
\sloppy{ The product automaton $P$ between the joint transition system $T$ and the B{\"u}chi automaton $B$ is defined as
{$\displaystyle
\begin{aligned} 
    \hspace{2cm} P := (S_P, S_{P,0}, E_P, F_P, w_p),
\end{aligned}
$ \par}
% $$P := (S_P, S_{P,0}, E_P, F_P, w_p)$$ 
    \noindent where (i) $S_P = S_T \times Q_B$, (ii) $S_{P,0}:= (s_0, q_0)$ is an initial state, (iii) $E_P \subseteq S_P \times S_P$, where $((s_i,q_k) ,(s_j,q_l)) \in E_P$ if and only if $(s_i, s_j)\in E_T$ and $\left(q_k, L_T\left(s_j\right),q_l\right) \in \delta_B$, (iv) $F_P := S_T \times Q_f $ set of final states, and (v) $w_P : E_P \rightarrow \mathbb{N}_{>0}$ such that $w_P((s_i,q_k) ,(s_j,q_l)) := w_T(s_i, s_j)$}. To generate a trajectory in $T$ which satisfies LTL query, we can refer $P$.
%\is{The sentence above is not clear.}\dg{Done}
Refer ~\cite{belta5650896} for examples.
\end{example}

==> Images/problem.tex <==
\section{Problem Definition} % Main chapter title
\label{sec-problem}

\sloppy Consider a team of robots represented as transition systems $\{ T_1,...,T_n\}$, moving in a static workspace $\mathcal{W}$ and their collective motion is modeled as a joint transition system $T$. A run over the transition system $T$ starting at initial state $s_0$ defines the trajectory of the robots in the $\mathcal{W}$.
Suppose, the robots are given a task in the form of an LTL query $\phi$ over $\Pi_T$ which needs to be completed collectively by them repetitively and infinitely many times. 
We construct a B{\"u}chi automaton $B$ from $\phi$. Let $\Pi_c = \{ c \:|\: c \in \Pi_B$ and $ \exists \delta_B(q_i , c) =  q_j$ where, $q_i \in Q_B$ and $q_j \in Q_f  \}$. Let $F_{\pi} = \{ s_i \: | \: s_i \in S_T$ and $ s_i \vDash \pi_j$ where $\pi_j \in \Pi_c \}$. $F_\pi$ represents a set of all the possible final states (final state is the last state in  the complete trajectory in $T$ which satisfies $\phi$) to be visited by the team on the path to complete the task. Our objective is to find the path in $T$(which represents the trajectories of the robots in $\mathcal{W}$) in the form of cycle with minimum cost and also which completes the task. Such path will always contain one of the states from $F_\pi$.

Let us assume that there exists at least one run over $T$ which satisfies $\phi$. Let $\mathcal{R} = s_0,s_1,s_2,...$ be an infinite length run/path over $T$ which satisfies $\phi$ and so there exists $f \in F_\pi$ which occurs on $\mathcal{R}$ infinitely many times. From $\mathcal{R}$, we can extract all the time instances at which $f$ occurs. Let $t_\mathcal{R}^f(i)$ denotes the time instance of $i^{th}$ occurrence of state $f$ on $\mathcal{R}$.
Our goal is to synthesize an infinite run $\mathcal{R}$ which satisfies the LTL formulae $\phi$  and minimizes the cost function 
\begin{equation} \label{eq1}
\mathcal{C}(\mathcal{R})=\limsup_{i \rightarrow+\infty} \sum_{k=t_\mathcal{R}^f(i)}^{t_\mathcal{R}^f(i+1)-1} w_T(s_k, s_{k+1})
\end{equation}

\subsection{Prefix-Suffix Structure} The accepting run  $\mathcal{R}$ of infinite length can be divided into two components namely  \emph{prefix} ($\mathcal{R}_{pre}$) and \emph{suffix} ($\mathcal{R}_{suf}$). A prefix is a finite run from initial state of the robot to an accepting state $f \in F_\pi$ and a suffix is a finite length run starting and ending at $f$ reached by the prefix, and containing no other occurrence of $f$. This suffix will be repeated periodically and infinitely many times to generate an infinite length run $\mathcal{R}$. So, we can represent run $\mathcal{R}$ as $\mathcal{R}_{pre}. \mathcal{R}_{suf}^\omega$, where $\omega$ denotes the suffix being repeated infinitely many times.

\noindent \emph{Lemma 3.1: }
For every run $\mathcal{R}$ which satisfies LTL formulae $\phi$ and minimizes cost function \eqref{eq1}, there exists a run $\mathcal{R}_c$ which satisfies $\phi$, minimizes cost function (\ref{eq1}) and is in prefix-suffix structure. Refer~\cite{belta5650896} for the proof. 

The cost of such run $\mathcal{R}_c$ is the cost of its suffix. So, now our goal translates to determining an algorithm which finds minimum cost suffix run starting and ending at a state $f \in F_\pi$ and having a finite length prefix run starting at initial state $s_0 \in S_T$ and ending at $f$. 
So, let $\mathcal{R} = \mathcal{R}_{pre}.\mathcal{R}_{suf}^\omega$, where $\mathcal{R}_{pre} = s_0,s_1,s_2,...,s_p$ be a prefix and $\mathcal{R}_{suf} = s_{p+1},s_{p+2},...,s_{p+r}$ be a suffix, where $s_{p+r} = s_p$. 
%\is{where $s_{p+r} = s_p$?}\dg{Done} 
We can redefine the cost function given in \ref{eq1} as
\begin{equation} \label{eq3}
 \mathcal{C}(\mathcal{R})= \mathcal{C}(\mathcal{R}_{suf}) = \sum_{i=p+1}^{p+r-1} w_T(s_i, s_{i+1})
\end{equation}
\begin{question}
Given a joint transition system $T$ capturing the motion of the team of robots in workspace $\mathcal{W}$ and an LTL formulae $\phi$ representing the task given to the robots, find an infinite length run $\mathcal{R}$ in prefix-suffix form over $T$ which minimizes the cost function \eqref{eq3}.
\end{question}

\noindent
%\smallskip
\textbf{Note:} If we want to deal with the LTL specifications that can be satisfied by the finite trajectories (for example, $\diamondsuit a$ or $a_1 U a_2$), we can define a cost function that captures the cost of the prefix, denoted by $\mathcal{C}(\mathcal{R}_{pre})$.
%\is{Dhaval: Please check.}\dg{It's correct}
% \dg{ In case of finite LTL specification, we can always consider the cost function to be a cost of prefix. In this case, the generated trajectories will be finite. i.e. from initial location to some final state.}
% \is{Comment on how to modify the cost function to deal with LTL formula leading to finite traces.}




\shortversion {
\subsection{Baseline Solution Approach}
The state-of-the-art solution to the above problem~\cite{UlusoySDBR13} uses the automata-theoretic  model  checking  approach.  It  computes  product automaton of $T$ and $B$ and then uses Dijkstra's shortest path algorithm to compute the required minimum cost suffix run having a valid prefix. 
The size of $T$ increases exponentially with the increase in the number of robots and also the workspace size. It consumes a huge amount of memory, which becomes an hindrance to scale up this algorithm.
In the next section, we present our algorithm \textsf{MT*} and use the algorithm proposed in~\cite{UlusoySDBR13} as the baseline for quantitative comparison. 
}
\longversion {
{\color{blue}
\subsection{Baseline Solution Approach}
The baseline solution to above problem uses the automata-theoretic model checking approach~\cite{UlusoySDBR13}, the steps of which are outlined in the Algorithm~\ref{baselineSolution}.

\begin{algorithm2e}
\SetAlgoLined
\DontPrintSemicolon
\setstretch{0.9}
\textbf{Input:} Transition systems $\{ T^1,...,T^n\}$, $\phi$: LTL formulae\;
\textbf{Output: }A set of runs $\{ \mathcal{R}^1,...,\mathcal{R}^n \}$that satisfies $\phi$\;
\BlankLine
Construct a joint transition system $T$\;
Convert $\phi$ to a B\"uchi automaton $B$\;
Compute the product automaton $P = T \times B$\;
\For{all $f \in F_P$ }{
$\mathcal{R}_f^{suf} \gets \mathtt{Dijkstra's\_Algorithm}(\: \emph{f} \:,\:  \emph{f}\:)$\;
$\mathcal{R}_f^{pre} \gets \mathtt{Dijkstra's\_Algorithm}(\: S_{P,0} \:,\:  \emph{f}\:)$
}
$\mathcal{R}_P^{suf} \gets$ minimum of all $\mathcal{R}_f^{suf}$ \;
$\mathcal{R}_P^{pre} \gets$ prefix of $\mathcal{R}_P^{suf}$ \;
$\mathcal{R}_P = \mathcal{R}_P^{suf} . \mathcal{R}_P^{pre} $\;
Project $\mathcal{R}_P$ over $T$ to compute $\mathcal{R}_T$\;
Project $\mathcal{R}_T$ over $\{ T^1,...,T^n\}$ to obtain runs $\{\mathcal{R}^1,...,\mathcal{R}^n\}$
\caption{Baseline\_Solution}
\label{baselineSolution}
\end{algorithm2e} 

The first step in this algorithm is to compute
the joint transition system $T$ from the transition systems of the individual robots $T^i$. Then we compute B\"uchi automaton from the given LTL query $\phi$. We then compute the product automaton of $T$ and $B$. In this product automaton, for each final state $f \in F_P$, we find a prefix run starting from initial state $S_{P,0}$ to $f \in F_P$ and then find minimum cost cycle starting and ending at $f$ using Dijkstra's algorithm. We then choose the prefix-suffix pair with the smallest $\mathcal{C}(\mathcal{R}_P)$ cost i.e. the pair with smallest suffix cost, and project it on $T$ to obtain the run $\mathcal{R}_T$ which represents the joint motion all the robots in $\mathcal{W}$. We then  project $\mathcal{R}_T$ over individual $T^i$ to obtain the  of the individual robots $\mathcal{R}^i$. The trajectory $\mathcal{R}^i$ for the $i$-th robot provides us with the cyclic trajectory which the robot can follow repetitively to complete the given task $\phi$ repetitively.  

% The cost to compute a joint transition system is exponential with respect to the number of robots n. Let $|\mathcal{W}|$ be the number of states in $\mathcal{W}$.
% Then, maximum number of states in the joint transition system $T$ can be $|\mathcal{W}|^n$.
% Let the total number of sub formulae in LTL formula $\Phi$ be denoted as $|\Phi|$. Thus, the maximum number of states in the automaton is $2^{|\Phi|}$. In this way, the LTL to B\"{u}chi automaton conversion has the computational complexity $\mathcal{O}(2^{|\Phi|})$ as mentioned in \cite{DuretLutz2004SPOTAE}. 
% We compute the product graph using the BFS algorithm. Thus, the complexity to compute the reduced graph is given as $\mathcal{O} (|S_P| + |E_P|)$. Since we run Dijkstra's algorithm for finding shortest suffix cycle for each point in $f \in F_P$, the complexity of do it is $\|F_P\| \times (\|E_{P}\| \times log \|S_{P}\|)$.
% So, the overall complexity of the baseline solution is $\mathcal{O}( 2 ^ {|\Phi|} + ( |S_P| + |E_P| ) + |F_P| * |E_P|*log|V_P| )$ . 
In the following section, we present MT$^*$ algorithm that provides a significantly improved running time for generating an optimal trajectory satisfying a given LTL query.
}
}

% The baseline solution to above problem uses the automata-theoretic model checking approach \cite{UlusoySDBR13}, the steps of which are outlined in the Algorithm~\ref{baselineSolution}.

% \begin{algorithm2e}
% \SetAlgoLined
% \DontPrintSemicolon
% \setstretch{0.9}
% \textbf{Input:} Transition systems $\{  T^1,...,T^n\}$, $\phi$: LTL formulae\;
% \textbf{Output: }A set of runs $\{  \mathcal{R}^1,...,\mathcal{R}^n \}$that satisfies $\phi$\;
% \BlankLine
% Construct a joint transition system $T$\;
% Convert $\phi$ to a B\"uchi automaton $B$\;
% Compute the product automaton $P = T \times B$\;
% \For{all $f \in F_P$ }{
% $\mathcal{R}_f^{suf} \gets \mathtt{Dijkstra's\_Algorithm}(\: \emph{f} \:,\:  \emph{f}\:)$\;
% $\mathcal{R}_f^{pre} \gets \mathtt{Dijkstra's\_Algorithm}(\: S_{P,0} \:,\:  \emph{f}\:)$
% }
% $\mathcal{R}_P^{suf} \gets$ minimum of all $\mathcal{R}_f^{suf}$ \;
% $\mathcal{R}_P^{pre} \gets$ prefix of $\mathcal{R}_P^{suf}$ \;
% $\mathcal{R}_P = \mathcal{R}_P^{suf} . \mathcal{R}_P^{pre} $\;
% Project $\mathcal{R}_P$ over $T$ to compute $\mathcal{R}_T$\;
% Project $\mathcal{R}_T$ over $\{  T^1,...,T^n\}$ to obtain runs $\{\mathcal{R}^1,...,\mathcal{R}^n\}$
% \caption{Baseline\_Solution}
% \label{baselineSolution}
% \end{algorithm2e} 

% The first step in this algorithm is to compute
% the joint transition system $T$ from the transition systems of the individual robots $T^i$. Then we compute B\"uchi automaton from the given LTL query $\phi$. We then compute the product automaton of $T$ and $B$. In this product automaton, for each final state $f \in F_P$, we find a prefix run starting from initial state $S_{P,0}$ to $f \in F_P$
% \is{$S_{P,0}$ is a set of states. We may mention somewhere that we assume that there is only one initial state.}
% and then find minimum cost cycle starting and ending at $f$ using Dijkstra's algorithm. We then choose the prefix-suffix pair with the smallest $\mathcal{C}(\mathcal{R}_P)$ cost i.e. the pair with smallest suffix cost, and project it on $T$ to obtain the run $\mathcal{R}_T$ which represents the joint motion all the robots in $\mathcal{W}$. We then  project $\mathcal{R}_T$ over individual $T^i$ to obtain the  of the individual robots $\mathcal{R}^i$. The trajectory $\mathcal{R}^i$ for the $i$-th robot provides us with the cyclic trajectory which the robot can follow repetitively to complete the given task $\phi$ repetitively.  

% The cost to compute a joint transition system is exponential with respect to the number of robots n. Let $|\mathcal{W}|$ be the number of states in $\mathcal{W}$.
% Then, maximum number of states in the joint transition system $T$ can be $|\mathcal{W}|^n$.
% Let the total number of sub formulae in LTL formula $\Phi$ be denoted as $|\Phi|$. Thus, the maximum number of states in the automaton is $2^{|\Phi|}$. In this way, the LTL to B\"{u}chi automaton conversion has the computational complexity $\mathcal{O}(2^{|\Phi|})$ as mentioned in \cite{DuretLutz2004SPOTAE}. 
% We compute the product graph using the BFS algorithm. Thus, the complexity to compute the reduced graph is given as $\mathcal{O} (|S_P| + |E_P|)$. Since we run Dijkstra's algorithm for finding shortest suffix cycle for each point in $f \in F_P$, the complexity of do it is $\|F_P\| \times (\|E_{P}\| \times log \|S_{P}\|)$.
% So, the overall complexity of the baseline solution is $\mathcal{O}( 2 ^ {|\Phi|} + ( |S_P| + |E_P| ) + |F_P| * |E_P|*log|V_P| )$ . 
% In the following section, we present \textsf{MT*} algorithm that provides a significantly improved running time for generating an optimal trajectory satisfying a given LTL query.

==> Images/related.tex <==
\section{Related Work}
\label{related}

Heuristic based search algorithms such as A* (for a single robot)~\cite{} and M* (for a multi-robot system)~\cite{} have been successfully applied to solving point-to-point path planning problems and are proven to be significantly faster than Dijkstra's shortest path algorithm.

Several researchers have studied the temporal logic path finding problem where specification requires the path to be finite in length
Multi-Agent Path Finding (MAPF) is a widely studied planning problem where the goal is to find collision-free paths for a number of agents from their initial locations to some specified goal locations~\cite{}. The MAPF problem is a special class of the finitel LTL path synthesis problem for multi-agent systems where the specification of each robot is given by the LTL formula ``eventually $goal$'', where $goal$ is the proposition that becomes true when the particular robot reaches its goal location. Like the work by Belta and ..., our focus in this paper is rather those LTL specifications that can be satisfied only by infinite trajectories represented by a prefix followed by a loop

Finite LTL

==> prelim.tex <==

\section{Preliminaries} % Main chapter title
\label{sec-preliminaries}


\subsection{Workspace, Robot Actions and Trajectory}
% The environments for robotic applications are continuous in nature. To reduce the amount of computation required during the motion planning of the robots in such environments, they are partitioned %discredited 
% into smaller cells or blocks based on the dynamics of the robot. We call it a \emph{discrete workspace} in this paper.
In this paper, we assume that a team of $n$ robots operates in a 2-D or a 3-D discrete workspace $\mathcal{W}$ which we represent as a grid map. The grid divides the workspace into square-shaped cells. Every cell in the workspace $\mathcal{W}$ can be referenced using its coordinates. Some cells in the grid can be marked as obstacles and cannot be visited by any robot. We denote the set of obstacles using $\mathcal{O}$.
We capture the motion of a robot using a set of actions $Act$. The robot changes its state in the workspace by performing the actions from $Act$. An action $act \in Act$ is associated with a $cost$, which captures the energy consumption or time delay (based on the need) to execute it. A robot can move to satisfy a given specification by executing a sequence of actions in $Act$ generating a \emph{trajectory} of states it attains. The \emph{cost of a trajectory} is the sum of costs of the actions to generate the trajectory. 

\subsection{Transition System}
We model the motion of the robot $i$ in the workspace $\mathcal{W}$ as a weighted transition system defined as
\mbox{$T^i := (S^i, s_0^i, E^i,\Pi^i, L^i, w^i),$}
% {
% $\displaystyle
% \begin{aligned}[c] 
% \hspace{2cm} T^i := (S^i, s_0^i, E^i,\Pi^i, L^i, w^i),
% \end{aligned}
% $ 
% \par}
% $T^i := (S^i, s_0^i, E^i,\Pi^i, L^i, w^i, \mathcal{O}^i )$ 
\noindent where (i) $S^i$ is the set of states,  
(ii) $s_0^i \in S^i$ is the initial state of the robot $i$,  (iii) $E^i \subseteq S^i \times S^i$ is the set of transitions/edges allowed to be taken by robot $i$, $(s_1^i , s_2^i) \in E^i$  iff  $s_1^i , s_2^i \in S^i$ and $s_1^i$ $\xrightarrow[]{act}$ $s_2^i$, where $act \in Act$,  (iv) $\Pi^i$ is the set of atomic propositions defined for robot $i$, (v) $L^i : S^i$ $\rightarrow$ $2^{\Pi^i}$ is a map which provides the set of atomic propositions satisfied at a state, (vi) $w^i: E^i$ $\rightarrow$ $\mathbb{N}_{>0}$ is a weight function.

%\is{The set of obstacles should not be part of the transition system of a robot.}\dg{Done}

\subsection{Joint Transition System}
A joint transition system $T$ is a transition system that captures the collective motion of a team of $n$ robots in a workspace$(\mathcal{W})$, where each robot executes one action from the set of actions $Act$ available to it. We define a joint transition system as
\mbox{$ T :=\: ( S_T,\; s_0,\; E_T,\; \Pi_T,\; L_T,\; w_T ),$}
% {
% $\displaystyle
% \begin{aligned}
%     \hspace{2cm} T :=\: ( S_T,\; s_0,\; E_T,\; \Pi_T,\; L_T,\; w_T ),
% \end{aligned}
% $ 
% \par}
% $T :=\: ( S_T,\; s_0,\; E_T,\; \Pi_T,\; L_T,\; w_T )$
%\noindent 
where (i) $S_T$ is the set of vertices/states in a joint transition system, where each vertex is of form $\langle s^1, s^2,...,s^n\rangle$, $s^i$ represents the state of robot $i$ in transition system $T^i$, (ii) $s_0:=\langle s^1_0, s^2_0,...,s^n_0\rangle  \in S_T$ is the joint initial state of the team of $n$ robots, (iii) $E_T \subseteq S_T \times S_T$ is the set of edges. $(s_1,s_2) \in E_T$ iff $s_1 , s_2 \in S_T$ and $(s_1^i,s_2^i) \in E^i$ for all $i \in \{ 1,2,...,n\}$, (iv) $\Pi^T := \bigcup_{i=1}^n \Pi^{i}$ is the set of atomic propositions, (v) $L_T :  S_T \rightarrow 2^{\Pi_T}$, and $L_T(s_{1}) := \bigcup_{i=1}^n L^i(s_{1}^i)$ gives us set of propositions true at state $s_1$, (vi) $w_T : E^T \rightarrow \mathbb{N}_{>0}$, and $w_T( s_{1}, s_{2} ) := \sum_{i=1}^n w^i(s_{1}^i, s_{2}^i)$ is a weight function.

We can also think of the transition system as a weighted directed graph with vertices, edges, and a weight function. Whenever we use some graph algorithm over a transition system, we mean to apply it over its equivalent graph. 


\begin{figure}[t] 
\centering
\subfigure[Workspace $\mathcal{W}$ with propositions $P_{1}, P_2 \text{ and } P_{3} $]{\centering \label{exampleGrid}\includegraphics[width=40mm]{Images/Map8x8.png}}
\hspace{2mm}
\subfigure[B\"{u}chi automaton B for query: $\square(\Diamond P_{1} \land \Diamond P_{2} \land \lnot P_{3})$]{\centering \label{exampleAutomata}\includegraphics[width=37mm]{Images/Autometa.png}}
\caption{Workspace $\mathcal{W}$ and B\"uchi Automaton}
\label{ws}
\end{figure}

\begin{example}

%\is{Could we draw the workspace so that the bottom-left corner becomes (0,0)? The current representation is not very intuitive.}\dg{Done}
Throughout this paper, we will use a warehouse pick-and-drop example for illustration purposes.
%Throughout this paper, we will use the workspace $\mathcal{W}$ shown in Figure \ref{exampleGrid} for the illustration purpose. 
The workspace $\mathcal{W}$ is shown in Figure \ref{exampleGrid}. 
We build a transition systems $T^i$ for all the robots over $\mathcal{W}$ where $\Pi^i = \Pi_T = \{ P_1, P_2 , P_3 \}$. The proposition $P_i$ is satisfied if the robot is at one of the locations denoted by $P_i$.
Here, $P_1$, $P_2$, and $P_3$ correspond to drop location, pickup location, and the locations to be avoided by the robots, respectively. Cells with black colour represent obstacles ($\mathcal{O}$).
We assume that from any cell in $\mathcal{W}$, a robot can move to one of its four neighbouring cells with cost $1$ or stay at the same location with cost $0$. 
\end{example}

\subsection{Linear Temporal Logic}
The path planning query/task in our work is given in terms of formulae written using \emph{Linear Temporal Logic} (LTL).
\sloppy{LTL formulae over the set of atomic propositions $\Pi_T$ are formed according to the following grammar~\cite{Baier:2008:PMC:1373322}:
{
$\displaystyle
\begin{aligned}[c] 
    \hspace{1cm} \phi:: = \mathtt{true} \;|\; a \;| \;\phi_{1} \land \phi_{2} \;|\; \neg\phi \;|\; X \phi \;|\; \phi_{1} U \phi_{2}.
\end{aligned}
$ 
\par}
% $$\Phi:: = \mathtt{true} \;|\; a \;| \;\phi_{1} \land \phi_{2} \;|\; \neg\phi \;|\; X \phi \;|\; \phi_{1} U \phi_{2} $$ 
The basic ingredients of an LTL formula are the atomic propositions $a \in \Pi_T$, the Boolean connectors like conjunction $\land$ and negation $\neg$, and two temporal operators $X$ (next) and $U$ (until). 
The semantics of an LTL formula is defined over an infinite trajectory $\sigma$. 
The trajectory $\sigma$ satisfies a formula $\xi$, if the first state of $\sigma$ satisfies $\xi$.
The logical operators conjunction $\land$ and negation $\neg$ have their usual meaning.
For an LTL formula $\phi$,
$X\phi$ is $\textsf{true}$ in a state if $\phi$ is satisfied at the next step. The formula $\phi_1 \ U \ \phi_2$ denotes that $\phi_1$ must remain $\textsf{true}$ until $\phi_2$ becomes $\textsf{true}$ at some point in future.
The other LTL operators that can be derived are  $\square$ (\emph{Always}) and $\Diamond$ (\emph{Eventually}). The formula $\square \phi$ denotes that $\phi$ must be satisfied all the time in the future. The formula $\Diamond \phi$ denotes that $\phi$ has to hold sometime in the future. We have denoted negation $\lnot P$ as $!P$ and conjunction as $\&$ in the Figures. }

\subsection{B{\"u}chi Automaton}
For any LTL formula $\phi$ over a set of propositions $\Pi_T$, we can construct a B{\"u}chi automaton with input alphabet $\Pi_B = 2^{\Pi_T}$. We can define a B{\"u}chi automaton as
% {
% $\displaystyle
% \begin{aligned} 
%     \hspace{2cm} {B:= (Q_B, q_0, \Pi_B, \delta_B, Q_f)},
% \end{aligned}
% $ \par}
\mbox{${B:= (Q_B, q_0, \Pi_B, \delta_B, Q_f)}$}, 
%\noindent 
where (i) $Q_B$ is a finite set of states, (ii) $q_0 \in Q_B$ is the initial state, (iii) $\Pi_B = 2^{\Pi_T}$ is the set of input symbols accepted by the automaton, (iv) $\delta_B \subseteq Q_B \times \Pi_B \times Q_B$ is a transition relation, and (v) $Q_f \subseteq Q_B$ is a set of final states.
An accepting state in the B\"uchi automaton is the one that needs to occur infinitely often on an infinite length string consisting of symbols from $\Pi_B$ to get accepted.

\begin{example}
Figure~\ref{exampleAutomata} shows the B\"uchi automaton for an LTL task $\square(\Diamond P_{1} \land \Diamond P_{2} \land \neg P_{3})$, which means that the robots should always repeat visiting pick up locations $P_2$ and drop location $P_1$, and always avoid locations $P_3$. Here, $q_0$ is the start state as well as the final state. It informally depicts the steps to be followed in order to compete the task $\phi$. The transitions $q_1 \rightarrow q_2 \rightarrow q_0$ leads us to visit a state 
where $P_1 \land \lnot P_2 \land \lnot P_3$ is satisfied by going through only those states which satisfy $\lnot P_1 \land \lnot P_3$ and then go to state where $P_2 \land \lnot P_3 $ is satisfied using states which  satisfy $\lnot P_2 \land \lnot P_3$. This way, we can also understand the meaning of the other transitions. 
\end{example}
% \dg{As per the analogy we used above, this LTL mission tell the robots to always and eventually visit pick up locations $P_2$ and drop location $P_1$ and always avoid locations $P_3$.}    

\subsection{Product Automaton}\label{productAutomaton}
\sloppy{ The product automaton $P$ between the joint transition system $T$ and the B{\"u}chi automaton $B$ is defined as
% {$\displaystyle
% \begin{aligned} 
%     \hspace{2cm} P := (S_P, S_{P,0}, E_P, F_P, w_p),
% \end{aligned}
% $ \par}
\mbox{$P := (S_P, S_{P,0}, E_P, F_P, w_p)$}, 
%\noindent 
    where (i) $S_P = S_T \times Q_B$, (ii) $S_{P,0}:= (s_0, q_0)$ is an initial state, (iii) $E_P \subseteq S_P \times S_P$, where $((s_i,q_k) ,(s_j,q_l)) \in E_P$ if and only if $(s_i, s_j)\in E_T$ and $\left(q_k, L_T\left(s_j\right),q_l\right) \in \delta_B$, (iv) $F_P := S_T \times Q_f $ set of final states, and (v) $w_P : E_P \rightarrow \mathbb{N}_{>0}$ such that $w_P((s_i,q_k) ,(s_j,q_l)) := w_T(s_i, s_j)$}. To generate a trajectory in $T$ which satisfies LTL query, we can refer $P$.
%\is{The sentence above is not clear.}\dg{Done}
Refer~\cite{belta5650896} for examples.


==> related.tex <==
\section{Related Work}
\label{related}

Heuristic based search algorithms such as A* (for a single robot)~\cite{} and M* (for a multi-robot system)~\cite{} have been successfully applied to solving point-to-point path planning problems and are proven to be significantly faster than Dijkstra's shortest path algorithm.

Several researchers have studied the temporal logic path finding problem where specification requires the path to be finite in length
Multi-Agent Path Finding (MAPF) is a widely studied planning problem where the goal is to find collision-free paths for a number of agents from their initial locations to some specified goal locations~\cite{}. The MAPF problem is a special class of the finite LTL path synthesis problem for multi-agent systems where the specification of each robot is given by the LTL formula ``eventually $goal$'', where $goal$ is the proposition that becomes true when the particular robot reaches its goal location. Like the work by Belta and ..., our focus in this paper is rather those LTL specifications that can be satisfied only by infinite trajectories represented by a prefix followed by a loop

Finite LTL
